The Shared Task on Gender Rewriting

In this paper, we present the results and findings of the Shared Task on Gender Rewriting, which was organized as part of the Seventh Arabic Natural Language Processing Workshop. The task of gender rewriting refers to generating alternatives of a given sentence to match different target user gender contexts (e.g., female speaker with a male listener, a male speaker with a male listener, etc.). This requires changing the grammatical gender (masculine or feminine) of certain words referring to the users. In this task, we focus on Arabic, a gender-marking morphologically rich language. A total of five teams from four countries participated in the shared task.

==> participants.tex <==
\begin{table}[ht]
\begin{center}
% \setlength{\tabcolsep}{2pt}
% \scalebox{0.85}{
\begin{tabular}{|l|l|}
\cline{1-2}
\textbf{Team} & \textbf{Affiliation} \\\hline
\textbf{Cairo Team} & Microsoft Egypt, Egypt \\\hline
\textbf{CasaNLP} & Archipel Cognitive; and Leyton, Morocco \\\hline
\textbf{Distinguishers} & Taif University; and Umm Alqura University, KSA \\\hline
\textbf{Qaddoumi} & New York University, USA \\\hline
\textbf{UDEL-NLP} & University of Delaware, USA \\\hline
\end{tabular}
% }
\end{center}
\caption{List of the five teams who participated in the gender rewriting shared task.}
\label{tab:teams}
\end{table}
 
 

 







 



==> results_dev.tex <==
\begin{table}[]
    \setlength{\tabcolsep}{1.3pt}
    \centering
    \begin{tabular}{|l|c|c|c|c|}
    \cline{1-5}
     \textbf{Team} & \textbf{P} & \textbf{R} & \textbf{F\textsubscript{0.5}} & \textbf{BLEU} \\\hline
        
         \textbf{Cairo Team} & 82.88 & 69.94 & 79.92 & 96.69 \\\hline
         \textbf{Distinguishers} & 57.3 & 56.2 & 57.1 & XX \\\hline
         \textbf{Qaddoumi} & XX & XX & XX & XX\\\hline
         \textbf{UDEL-NLP} & XX & XX & XX  & XX \\\hline\hline
         \textbf{\newcite{alhafni-etal-2022-user}} & 88.67 & 86.84  & 88.30 & 98.05 \\\hline
         
    \end{tabular}
    \caption{Results on the DEV set of {\APGC} v2.1.}
    \label{tab:my_label}
\end{table}

==> sent_level_orig_stats.tex <==
\begin{table}[ht]
\setlength{\tabcolsep}{2.5pt}
\begin{center}
% \setlength{\tabcolsep}{2pt}
\scalebox{0.85}{
\begin{tabular}{|ll|c|ccc|}
\cline{1-6}
\multicolumn{2}{|c|}{\textbf{Sentences}} & \textbf{Label} & \multicolumn{3}{|c|}{\textbf{Rewriting Label}}\\\hline
2,818 & 56.4\% & B & & & \\\hline\hline
91 & 1.8\% & 1F/B & & 1M/B & \\\hline
172 & 3.4\% & 1M/B & & 1F/B & \\\hline\hline
559 & 11.2\% & B/2F & & B/2M & \\\hline
1,292 & 25.8\% & B/2M & & B/2F & \\\hline\hline
8 & 0.2\% & 1F/2F & 1M/2F & 1F/2M & 1M/2M \\\hline
21 & 0.4\% & 1F/2M & 1M/2F & 1F/2F & 2M/1F \\\hline
13 & 0.5\% & 1M/2F & 1F/2M & 1F/2M & 1F/2M \\\hline
26 & 1.4\% & 1M/2M & 1F/2M & 1M/2F & 1F/2F \\\hline
5,000 & & \multicolumn{4}{l}{} \\\cline{1-2}

\end{tabular}
}
\end{center}
\caption{Sentence-level statistics of the blind test set.}
\label{tab:sentence-level-stats-original}
\end{table}

==> sent_level_stats.tex <==
% \begin{table*}[t!]
% \begin{center}
% \setlength{\tabcolsep}{2.5pt}
% \scalebox{0.8}{
% \begin{tabular}{|c|c|c|c|c|ll|}
% \cline{1-7}
% \bf Input & \bf Target 1M/2M &  \bf Target 1F/2M & \bf \bf Target 1M/2F &  \bf \bf Target 1F/2F & \multicolumn{2}{c|}{\bf Sentences} \\\cline{1-7}


%     B & B & B & B &  B & 2,818 &  38.5\% \\\hline\hline
    
%     1F/B & 1M/B &  1F/B & 1M/B &  1F/B &  263 &  3.6\% \\\cline{1-7}
%     1M/B & 1M/B &  1F/B & 1M/B &  1F/B &  263 &  3.6\% \\\hline\hline

%     B/2F & B/2M &  B/2M  & B/2F &  B/2F & 1,851 & 25.3\% \\\cline{1-7}
%     B/2M & B/2M &  B/2M  & B/2F &  B/2F & 1,851 & 25.3\% \\\hline\hline
    
%     1F/2F & 1M/2M &  1F/2M & 1M/2F &  1F/2F & 68 & 0.9\% \\\cline{1-7}
%     1F/2M & 1M/2M &  1F/2M & 1M/2F &  1F/2F & 68 & 0.9\% \\\cline{1-7}
%     1M/2F & 1M/2M & 1F/2M & 1M/2F & 1F/2F &  68 &  0.9\% \\\cline{1-7}
%     1M/2M & 1M/2M & 1F/2M & 1M/2F & 1F/2F & 68  & 0.9\% \\\cline{1-7}

%     \multicolumn{5}{c|}{} & 7,318 &  \\\cline{6-7}

% \end{tabular}
% }
% \end{center}
% \caption{Sentence-level statistics of the balanced blind test set.}
% \label{tab:sentence-level-stats-balanced}
% \end{table*}


\begin{table*}[t!]
\begin{center}
\setlength{\tabcolsep}{2.2pt}
\scalebox{0.78}{

\begin{tabular}{|rr|c|ccc|  ccc  |c|c|c|c|c|rr|}
\multicolumn{2}{c}{} & \multicolumn{4}{c}{\bf(a)} & & & \multicolumn{6}{c}{\bf (b)} & \multicolumn{1}{c}{} \\
\cline{3-6}\cline{10-14}
\multicolumn{2}{c|}{}& \multicolumn{4}{c|}{\bf Original Test Set} & & & & \multicolumn{5}{c|}{\bf Balanced Test Set} & \multicolumn{2}{c}{} \\\cline{1-6}\cline{10-16}

\multicolumn{2}{|c|}{\bf Sentences} & \bf  Label &  \multicolumn{3}{c|}{\bf Rewriting Label}   &  & & &  \bf Input & \bf \bf Target 1M/2M &  \bf Target 1F/2M & \bf \bf Target 1M/2F &  \bf \bf Target 1F/2F & \multicolumn{2}{c|}{\bf Sentences} \\\cline{1-6}\cline{10-16}


    2,818 & 56.4\% & B &  & & & & & & B & B & B & B &  B & 2,818 &  38.5\%\\\hhline{*{6}{=}*{3}{~}*{7}{=}}
    
    91 & 1.8\% & 1F/B &  & 1M/B & & & & & 1F/B & 1M/B &  1F/B & 1M/B &  1F/B &  263 &  3.6\%\\\cline{1-6}\cline{10-16}
    172 & 3.4\% & 1M/B &  & 1F/B & & & & & 1M/B & 1M/B &  1F/B & 1M/B &  1F/B &  263 &  3.6\% \\\hhline{*{6}{=}*{3}{~}*{7}{=}}

    559 & 11.2\% & B/2F &  & B/2M & &  & & & B/2F & B/2M &  B/2M  & B/2F &  B/2F & 1,851 & 25.3\%\\\cline{1-6}\cline{10-16}
    1,292 & 25.8\% & B/2M &  & B/2F & &  & & & B/2M & B/2M &  B/2M  & B/2F &  B/2F &  1,851 & 25.3\% \\\hhline{*{6}{=}*{3}{~}*{7}{=}}
    
     8 & 0.2\%  & 1F/2F &  1M/2F & 1F/2M & 1M/2M & & & & 1F/2F & 1M/2M &  1F/2M & 1M/2F &  1F/2F & 68 & 0.9\% \\\cline{1-6}\cline{10-16}
     21 & 0.4\% & 1F/2M &  1M/2M & 1F/2F & 1M/2F & & & & 1F/2M & 1M/2M &  1F/2M & 1M/2F &  1F/2F &   68 & 0.9\% \\\cline{1-6}\cline{10-16}
     13 & 0.5\% & 1M/2F &  1F/2F & 1M/2M & 1F/2M & & & & 1M/2F & 1M/2M & 1F/2M & 1M/2F & 1F/2F &   68 & 0.9\% \\\cline{1-6}\cline{10-16}
     26 & 1.4\%& 1M/2M &  1F/2M & 1M/2F & 1F/2F & & & & 1M/2M & 1M/2M & 1F/2M & 1M/2F & 1F/2F &   68 & 0.9\% \\\cline{1-6}\cline{10-16}

     5,000 & & \multicolumn{4}{c}{} & & &   \multicolumn{6}{c|}{} & 7,318 & \\\cline{1-2}\cline{15-16}

\end{tabular}
}
\end{center}
\caption{Sentence-level statistics of the original (a) and the balanced test set (b) with its five versions.}
\label{tab:sentence-level-stats}
\end{table*}


